ML-based Fault Injection for Autonomous Vehicles: A Case for Bayesian Fault Injection

The safety and resilience of fully autonomous vehicles (AVs) are of significant concern, as exemplified by several headline-making accidents. While AV development today involves verification, validation, and testing, end-to-end assessment of AV systems under accidental faults in realistic driving scenarios has been largely unexplored. This paper presents DriveFI, a machine learning-based fault injection engine, which can mine situations and faults that maximally impact AV safety, as demonstrated on two industry-grade AV technology stacks (from NVIDIA and Baidu). For example, DriveFI found 561 safety-critical faults in less than 4 hours. In comparison, random injection experiments executed over several weeks could not find any safety-critical faults

==> 07000-discussion.tex <==
\section{Discussion}\label{ref:discussion}

\textbf{Simulate one timestep ahead instead of predicting velocity using Bayesian approach}\\

\textbf{Limitation of the Bayesian modeling}\\



==> Makefile <==
# ACG stolen from amagela (AMA)
#This Makefile builds: congestion
#
# THE FOLLOWING TARGETS ARE GENERALLY AVAILABLE
# all:                Performs all tasks to clean, build, and install the application and documentation
# spellcheckaspell:   This runs a spell checker on all TeX files within doc/
# spellcheckhunspell: This runs a spell checker on all TeX files within doc/
# clean:              Delete the files generated from building the examples and documentation
# purge:              This does clean and also removes the resultant document
# tar:                Create a stamped, Gzip-compressed tarball within directory tar

###### USER SETTINGS ######
# TITLE:      Name of resultant documentation
TITLE:=main

###### COMPILER SETTINGS (ONLY ADMINS BELOW) ######
#COMPILERS/LINKERS
#MAKPDF:=pdflatex  --shell-escape
#MAKPDF:=pdflatex  -lualatex
MAKPDF:=latexmk -pdf
CLEAN:=latexmk -c
PURGE:=latexmk -C

SPELLCHECKTARGET:=spellcheckaspell
ifeq ($(wildcard /usr/bin/hunspell),/usr/bin/hunspell)
	SPELLCHECKTARGET:=spellcheckhunspell
endif
ifeq ($(wildcard /opt/local/bin/hunspell),/opt/local/bin/hunspell)
	SPELLCHECKTARGET:=spellcheckhunspell
endif

#EXTRA VARS
LOGAPPEND:=$(shell date '+%Y%m%d_%H%M%S')

###### TARGETS ######
default: initpurge pdf clean
#ACG perfers to call clean separately
#default: initpurge pdf
pdf: $(TITLE).pdf
$(TITLE).pdf: $(TITLE).tex
%.pdf: %.tex
#	$(MAKPDF) >$*.build.log 2>&1 $<
	$(MAKPDF) $<

.PHONY: clean
clean:
	$(CLEAN)
	-find . -type f -name "*.bbl" -exec rm -f '{}' \;
	-find . -type f -name "*~" -exec rm -f '{}' \;
	-find . -type f -name "*.swp" -exec rm -f '{}' \;
	-find . -type f -name ".*~" -exec rm -f '{}' \;
	-find . -type f -name ".*.swp" -exec rm -f '{}' \;

#ACG added to get rid of pdf but not break the other calls
#.PHONY: veryclean
#veryclean: clean
#	$(VERYCLEAN)
#	-rm $(TITLE).pdf

.PHONY: initpurge
initpurge:
	-rm -f $(TITLE).pdf

.PHONY: purge
purge: clean
	$(PURGE)

.PHONY: spellcheckaspell
spellcheckaspell:
	-find . -type f -name "[0-9]*.tex" -exec aspell -c '{}' --lang=en_US --mode=tex \;

.PHONY: spellcheckhunspell
spellcheckhunspell:
	-find . -type f -name "[0-9]*.tex" -exec hunspell -t -d en_US '{}' \;

.PHONY: spellcheck
spellcheck: $(SPELLCHECKTARGET)

.PHONY: tar
tar: clean
	mkdir -p tar
	tar -czhf tar/$(TITLE)_$(LOGAPPEND).tgz $(TITLE).pdf Makefile *.tex *.bib figs

